Spin nematics, valence-bond solids and spin liquids in SO($N$) quantum spin models on the triangular lattice

We introduce a simple model of SO($N$) spins with two-site interactions which is amenable to quantum Monte-Carlo studies without a sign problem on non-bipartite lattices. We present numerical results for this model on the two-dimensional triangular lattice where we find evidence for a spin nematic at small $N$, a valence-bond solid (VBS) at large $N$ and a quantum spin liquid at intermediate $N$. By the introduction of a sign-free four-site interaction we uncover a rich phase diagram with evidence for both first-order and exotic continuous phase transitions.

==> dimertriplaq.latex <==
\setlength{\unitlength}{3158sp}%
%
\begingroup\makeatletter\ifx\SetFigFont\undefined%
\gdef\SetFigFont#1#2#3#4#5{%
  \reset@font\fontsize{#1}{#2pt}%
  \fontfamily{#3}\fontseries{#4}\fontshape{#5}%
  \selectfont}%
\fi\endgroup%
\begin{picture}(282,173)(535,-171)
\thinlines
\special{ps: gsave 0 0 0 setrgbcolor}\multiput(720,-10)(1.54799,-2.57998){58}{\makebox(2.0833,14.5833){\SetFigFont{5}{6}{\rmdefault}{\mddefault}{\updefault}.}}
\special{ps: grestore}\special{ps: gsave 0 0 0 setrgbcolor}\multiput(805,-158)(-3.00000,0.00000){58}{\makebox(2.0833,14.5833){\SetFigFont{5}{6}{\rmdefault}{\mddefault}{\updefault}.}}
\special{ps: grestore}\special{ps: gsave 0 0 0 setrgbcolor}\multiput(718,-10)(-1.55263,-2.58772){58}{\makebox(2.0833,14.5833){\SetFigFont{5}{6}{\rmdefault}{\mddefault}{\updefault}.}}
\special{ps: grestore}\special{ps: gsave 0 0 0 setrgbcolor}\multiput(718,-10)(-3.00000,0.00000){58}{\makebox(2.0833,14.5833){\SetFigFont{5}{6}{\rmdefault}{\mddefault}{\updefault}.}}
\special{ps: grestore}\special{ps: gsave 0 0 0 setrgbcolor}\multiput(548,-10)(1.55263,-2.58772){58}{\makebox(2.0833,14.5833){\SetFigFont{5}{6}{\rmdefault}{\mddefault}{\updefault}.}}
\special{ps: grestore}\end{picture}

